iDARTS: Differentiable Architecture Search with Stochastic Implicit Gradients

\textit{Differentiable ARchiTecture Search} (DARTS) has recently become the mainstream of neural architecture search (NAS) due to its efficiency and simplicity. With a gradient-based bi-level optimization, DARTS alternately optimizes the inner model weights and the outer architecture parameter in a weight-sharing supernet. A key challenge to the scalability and quality of the learned architectures is the need for differentiating through the inner-loop optimisation. While much has been discussed about several potentially fatal factors in DARTS, the architecture gradient, a.k.a. hypergradient, has received less attention. In this paper, we tackle the hypergradient computation in DARTS based on the implicit function theorem, making it only depends on the obtained solution to the inner-loop optimization and agnostic to the optimization path. To further reduce the computational requirements, we formulate a stochastic hypergradient approximation for differentiable NAS, and theoretically show that the architecture optimization with the proposed method, named iDARTS, is expected to converge to a stationary point. Comprehensive experiments on two NAS benchmark search spaces and the common NAS search space verify the effectiveness of our proposed method. It leads to architectures outperforming, with large margins, those learned by the baseline methods.

==> backup.tex <==
\section{The full results of Ablation study on NAS-Bench-201}



\begin{table*}[ht]
\footnotesize
\centering
\caption{Comparison results with different $\gamma$ on NAS-Bench-201. %``*" indicates that we reproduce the results with same random seeds as our approaches.
}
\begin{tabular}
{|l|c|c|c|c|c|c|c|c|}
\hline

\makecell[c]{\multirow{2}*{Method}}&\multicolumn{2}{c|}{CIFAR-10}&\multicolumn{2}{c|}{CIFAR-100}&\multicolumn{2}{c|}{ImageNet-16-120}\\
~&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%)}&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%) }&\multicolumn{1}{c}{Valid(\%) }&\multicolumn{1}{c|}{Test(\%)}\\
\hline
\hline
%Random baseline\cite{xie2018snas}&64.1&61.5&23&-&Single path&random\\
%NAS\shortcite{zoph2016neural}&-&64&25&1e$^{4}$&Single path&RL\\
iDARTS ($\gamma$=0.05)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($\gamma$=0.02)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($\gamma$=0.01)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($\gamma$=0.005)&\textbf{91.52$\pm$0.09}&\textbf{94.33$\pm$0.04}&\textbf{72.67$\pm$0.08}&\textbf{72.95$\pm$0.27}&\textbf{45.39$\pm$0.17}&\textbf{46.32$\pm$0.39}\\
iDARTS ($\gamma$=0.001)&\textbf{91.52$\pm$0.09}&\textbf{94.33$\pm$0.04}&\textbf{72.67$\pm$0.08}&\textbf{72.95$\pm$0.27}&\textbf{45.39$\pm$0.17}&\textbf{46.32$\pm$0.39}\\
\hline
\end{tabular}
\flushleft{DARTS* sets the search epochs to 30, so as our BaLeNAS. The best single run of our BaLeNAS (with \textit{random seed 100} or \textit{101}) achieves \textbf{94.37\%}, \textbf{73.22\%}, and \textbf{46.71\%} test accuracy on CIFAR-10, CIFAR-100, and ImageNet, respectively.}
\label{tab:}
\end{table*}


\begin{table*}[ht]
\footnotesize
\centering
\caption{Comparison results with different $T$ on NAS-Bench-201. %``*" indicates that we reproduce the results with same random seeds as our approaches.
}
\begin{tabular}
{|l|c|c|c|c|c|c|c|c|}
\hline

\makecell[c]{\multirow{2}*{Method}}&\multicolumn{2}{c|}{CIFAR-10}&\multicolumn{2}{c|}{CIFAR-100}&\multicolumn{2}{c|}{ImageNet-16-120}\\
~&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%)}&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%) }&\multicolumn{1}{c}{Valid(\%) }&\multicolumn{1}{c|}{Test(\%)}\\
\hline
\hline
%Random baseline\cite{xie2018snas}&64.1&61.5&23&-&Single path&random\\
%NAS\shortcite{zoph2016neural}&-&64&25&1e$^{4}$&Single path&RL\\
iDARTS ($T$=1)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($T$=2)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($T$=3)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($T$=4)&\textbf{91.52$\pm$0.09}&\textbf{94.33$\pm$0.04}&\textbf{72.67$\pm$0.08}&\textbf{72.95$\pm$0.27}&\textbf{45.39$\pm$0.17}&\textbf{46.32$\pm$0.39}\\
iDARTS ($T$=5)&\textbf{91.52$\pm$0.09}&\textbf{94.33$\pm$0.04}&\textbf{72.67$\pm$0.08}&\textbf{72.95$\pm$0.27}&\textbf{45.39$\pm$0.17}&\textbf{46.32$\pm$0.39}\\
\hline
\end{tabular}
\flushleft{DARTS* sets the search epochs to 30, so as our BaLeNAS. The best single run of our BaLeNAS (with \textit{random seed 100} or \textit{101}) achieves \textbf{94.37\%}, \textbf{73.22\%}, and \textbf{46.71\%} test accuracy on CIFAR-10, CIFAR-100, and ImageNet, respectively.}
\label{tab:}
\end{table*}

\begin{equation} \label{eq:}
\nabla_{\alpha}\mathcal{L}_{val}=(\frac{\partial \mathcal{L}_{val}}{\partial \alpha}+\frac{\partial \mathcal{L}_{val}}{\partial w}\frac{\partial w^*(\alpha)}{\partial \alpha})
\end{equation}

\begin{equation} \label{eq:}
w^*(\alpha)=w-\xi \nabla_{w}\mathcal{L}_{train}
\end{equation}

\begin{equation} \label{eq:}
\frac{\partial w^*(\alpha)}{\partial \alpha}=-\xi \frac{\partial^2 \mathcal{L}_{train}}{\partial \alpha \partial w}
\end{equation}



\begin{equation} \label{eq:}
\nabla_{\alpha}\mathcal{L}_{val}=(\frac{\partial \mathcal{L}_{val}}{\partial \alpha}-\xi \frac{\partial \mathcal{L}_{val}}{\partial w}\frac{\partial^2 \mathcal{L}_{train}}{\partial \alpha \partial w})
\end{equation}


$\theta\sim \mathcal{N}(\theta\mid \mu,\sigma^2)$  $\alpha_\theta$

%In this paper, we further make a reasonable assumption: in the last K steps, $w$ has reached the optimal $w^*$, which means that $w$ remains the same in the last K steps. In this way, after leverage the $h_{T-K}$, we could have our approximated hypergradient:
%\begin{equation} \label{eq:k_step_same}
%\begin{aligned}
%&h_K=\frac{\partial \mathcal{L}_2}{\partial \alpha}+\frac{\partial \mathcal{L}_2}{\partial w_T}Z_T\\
%&=\frac{\partial \mathcal{L}_2}{\partial \alpha}+\frac{\partial \mathcal{L}_2}{\partial w_T}B_{T}(\sum_{t=0}^{K}A_T^t).\\
%end{aligned}
%\end{equation}















\section{Concerns of our $h_K$}

Since we need to make the inner optimization achieves the optimal in the last K steps, we need a large T. However, this will greatly increase the training time. We utilized the weight sharing paradigm. 



1. The initialized supernet training equals to $S$ step of model training for every architecture. We could utilize the pre-training method to reduce the training time. $T-K$ step of training is enough to push an architecture to the optimal, which means in the last $K$ step, weights is nearly optimal.

2. In the early stage, the hypergradient is not accurate, we could consider a strong noise term in the architecture optimization, and reduce it during the architecture search. Or,we could uses a large T in the early stage, and a smaller T in the later stage.

3. A variant: consider the ``Meta-Learning with Implicit Gradients" \cite{rajeswaran2019meta} and WPL, with overcoming forgetting. controlling the strength of the prior ($\theta$) relative to the data ($\mathcal{D}$).


\textbf{Scope and Limitations.}

\section{Introduction of Weighted Softmax (maybe in the appendix)}

As we discussed, the depth regularization maybe useless in the differentiable NAS, since the softmax is applied in each connection. To account the depth information, we try to use a Weighted-Softmax. In our consideration, we hope the softmax would not remove the effect of the softmax. 
\begin{equation} \label{eq:softmax}
\bar{o}^{i,j}=\sum_{o\in \mathcal{O}}\frac{\textup{exp}(\alpha_{o}^{(i,j)})}{\sum_{o'\in \mathcal{O}}\textup{exp}(\alpha_{o'}^{(i,j)})}o(x)
\end{equation}


Since the forward of supernet training, DARTS uses the weighted operation, and the weights are calculated from the softmax. In our assumption, we hope all operation in some connection should not be encouraged. We can find that in DARTS, the $\frac{\textup{exp}(\alpha_{o}^{(i,j)})}{\sum_{o'\in \mathcal{O}}\textup{exp}(\alpha_{o'}^{(i,j)})}$ is the weight for each operation in each connection.

Now, let's simply take the $w_c=\sum_{o'\in \mathcal{O}}\textup{exp}(\alpha_{o'}^{(i,j)})$ as the weight of each connection, and we can use the $w'_c=\textup{softmax}(w_c)$ as the weight of each connection for the forward.



\section{Interesting Finding}
 With the progress of architecture search, the searched architecture is smaller and smaller.
 
 Need to calculate the gradient confusion for each operation.
 
 Need to set a pre-trained model, with only several step for architecture search. 
 
\section{Paper framework}

First introduce DARTS, and its one-step approximation. Then argue that 1-step is not enough, and we need to consider the T-step optimization, and than give the T-step formulation.

Then give the implicit differentiable function, and introduce the need to calculate the inverse of Hessian. Give several examples of approximation, including identity, fisher information matrix (only the diagonal element). And the Neumann series.

In this paper, we consider the Neumann series as approximation, and try to make the last K step are in the optimal point $w*$. In this way, our method could be seen as the first K term of T-step exact gradient.

In the first stage, we introduce the strong noise term (exploration) into the architecture optimization, since the gradient is not very accurate. In the late, we reduce the noise term.


Regularization, if necessary (``Meta-Learning with Implicit Gradients").


We first define the noise term $\varepsilon$ between the stochastic gradient $\nabla_{\alpha}\mathcal{L}_2^i(w^j(\alpha),\alpha)$ and the true gradient $\nabla_{\alpha}\mathcal{L}_2$ as:
\begin{equation} \nonumber
\varepsilon_{i,j}=\nabla_{\alpha}\mathcal{L}_2-\nabla_{\alpha}\mathcal{L}_2^i(w^j(\alpha_m),\alpha_m),
\end{equation}
and the error between the approximated gradient $\nabla_{\alpha}\mathcal{L}_2^{'}$ and the true gradient $\nabla_{\alpha}\mathcal{L}_2$ is defined as:
\begin{equation} \nonumber
e=\nabla_{\alpha}\mathcal{L}_2-\nabla_{\alpha}\mathcal{L}_2^{'},
\end{equation}
and we have:
\begin{equation} \nonumber
\nabla_{\alpha}\mathcal{L}_2=\nabla_{\alpha}\mathcal{L}_2^{'i}(w^j(\alpha),\alpha)+e+\varepsilon_{i,j},
\end{equation}
where we assume the approximation error $e$ and the noise $\varepsilon$ are orthogonal.




\begin{table*}[t]
\centering
\caption{Comparison results with different $T$ on NAS-Bench-201. %``*" indicates that we reproduce the results with same random seeds as our approaches.
}
\begin{tabular}
{|l|c|c|c|c|c|c|c|c|}
\hline

\makecell[c]{\multirow{2}*{Method}}&\multicolumn{2}{c|}{CIFAR-10}&\multicolumn{2}{c|}{CIFAR-100}&\multicolumn{2}{c|}{ImageNet-16-120}\\
~&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%)}&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%) }&\multicolumn{1}{c}{Valid(\%) }&\multicolumn{1}{c|}{Test(\%)}\\
\hline
\hline
%Random baseline\cite{xie2018snas}&64.1&61.5&23&-&Single path&random\\
%NAS\shortcite{zoph2016neural}&-&64&25&1e$^{4}$&Single path&RL\\
iDARTS ($T$=1)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($T$=2)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($T$=3)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($T$=4)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($T$=5)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
\hline
%iDARTS ($\gamma_\alpha$=0.01)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($\gamma_\alpha$=0.005)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($\gamma_\alpha$=0.002)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($\gamma_\alpha$=0.001)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($\gamma_\alpha$=0.0003)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
iDARTS ($\gamma_\alpha$=0.0001)&91.03$\pm$0.15&93.62$\pm$0.12&13.37$\pm$2.35&13.96$\pm$2.33&15.06$\pm$1.95&14.84$\pm$2.10\\
\hline
\end{tabular}
\label{tab:}
\end{table*}


\begin{figure}
 \subfloat[Validation error]{
  \begin{minipage}{4.2cm}
      \includegraphics[width=4.2cm,height=2.9cm]{figures/NAS+Bench+1Shot1+DARTS.pdf}
  \end{minipage}
 }
  \subfloat[Test errors]{
  \begin{minipage}{4.2cm}
       \includegraphics[width=4.2cm,height=2.9cm]{figures/NAS+Bench+1Shot1+DARTS+V2.pdf}
  \end{minipage} 
  }
 \caption{Validation and test error of iDARTS with different $K$ on the search space 3 of NAS-Bench-1Shot1. }
 \label{fig:K_nas1shot1}
\end{figure}


\begin{table*}[ht]
\footnotesize
\centering
\caption{Comparison results with different $\gamma$ on NAS-Bench-201. %``*" indicates that we reproduce the results with same random seeds as our approaches.
}
\begin{tabular}
{|l|c|c|c|c|c|c|c|c|}
\hline

\makecell[c]{\multirow{2}*{Method}}&\multicolumn{2}{c|}{CIFAR-10}&\multicolumn{2}{c|}{CIFAR-100}&\multicolumn{2}{c|}{ImageNet-16-120}\\
~&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%)}&\multicolumn{1}{c}{Valid(\%)}&\multicolumn{1}{c|}{Test(\%) }&\multicolumn{1}{c}{Valid(\%) }&\multicolumn{1}{c|}{Test(\%)}\\
\hline
\hline
%Random baseline\cite{xie2018snas}&64.1&61.5&23&-&Single path&random\\
%NAS\shortcite{zoph2016neural}&-&64&25&1e$^{4}$&Single path&RL\\
iDARTS ($\gamma$=0.05)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($\gamma$=0.05)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($\gamma$=0.02)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($\gamma$=0.01)&91.03$\pm$0.15&93.62$\pm$0.12&70.88$\pm$0.60&70.98$\pm$0.41&45.19$\pm$0.75&45.25$\pm$0.86\\
iDARTS ($\gamma$=0.005)&\textbf{91.52$\pm$0.09}&\textbf{94.33$\pm$0.04}&\textbf{72.67$\pm$0.08}&\textbf{72.95$\pm$0.27}&\textbf{45.39$\pm$0.17}&\textbf{46.32$\pm$0.39}\\
iDARTS ($\gamma$=0.001)&\textbf{91.52$\pm$0.09}&\textbf{94.33$\pm$0.04}&\textbf{72.67$\pm$0.08}&\textbf{72.95$\pm$0.27}&\textbf{45.39$\pm$0.17}&\textbf{46.32$\pm$0.39}\\
\hline
\end{tabular}
%\flushleft{DARTS* sets the search epochs to 30, so as our BaLeNAS. The best single run of our BaLeNAS (with \textit{random seed 100} or \textit{101}) achieves \textbf{94.37\%}, \textbf{73.22\%}, and \textbf{46.71\%} test accuracy on CIFAR-10, CIFAR-100, and ImageNet, respectively.}
\label{tab:}
\end{table*}

and we have
\begin{equation} \label{eq:}
\begin{aligned}
e_m \cdot \nabla_{\alpha}\mathcal{L}_2^{'}(w^*(\alpha_{m}),\alpha_{m}) &\geq -\frac{C_{\mathcal{L}_1^{w\alpha}}\ C_{\mathcal{L}_2^w}\ (1-\gamma \alpha )^{K+1}}{\alpha L_{\nabla_{\alpha}\mathcal{L}_2}^{'} } \left \|  \nabla_{\alpha}\mathcal{L}_2^{'}(w^*(\alpha_{m}),\alpha_{m}) \right \|^2\\
&=P \left \|  \nabla_{\alpha}\mathcal{L}_2^{'}(w^*(\alpha_{m}),\alpha_{m}) \right \|^2
\end{aligned}
\end{equation}



\textbf{Approximation 1:} Although the Hessian-vector produce is a practical solution for the implementation of calculating $\frac{\partial \mathcal{L}_2}{\partial w} \frac{\partial^2 \mathcal{L}_1}{\partial w\partial w}$, while its computation cost and memory requirement also increase with $K$, making it impractical for the architecture search in the DARTS search space. Another option, which has already been proven effective on large neural networks by several recent works \cite{kirkpatrick2017overcoming,pascanu2013revisiting,benyahia2019overcoming}, is to assume model weights are independent, and the Hessian $\frac{\partial^2 \mathcal{L}_1}{\partial w\partial w}$ could be approximated by a diagonal matrix the second order derivative $\frac{\partial^2 \mathcal{L}_1}{\partial w^2}$ when calculate the $\frac{\partial \mathcal{L}_2}{\partial w}\sum_{k=0}^{K}\left [ I- \gamma \frac{\partial^2 \mathcal{L}_1}{\partial w\partial w} \right ]^k$. This paper consider this approximation for the practical and efficient implementation since it only needs to calculate $\frac{\partial^2 \mathcal{L}_1}{\partial w^2}$ with a single step of back-propagation, which is very efficient without increasing too much memory consumption. We empirically found that this approximation still achieves competitive or even better performance in the three different NAS search space.
